Enumerating singular curves on surfaces

We enumerate the singular algebraic curves in a complete linear system on a smooth projective surface. The system must be suitably ample in a rather precise sense. The curves may have up to eight nodes, or a triple point of a given type and up to three nodes. The curves must also pass through appropriately many general points. The number of curves is given by a universal polynomial in four basic Chern numbers. To justify the enumeration, we make a rudimentary classification of the types of singularities using Enriques diagrams, obtaining results like Arnold's. We show that the curves in question do, in fact, appear with multiplicity 1 using the versal deformation space, Shustin's codimension formula, and Gotzmann's regularity theorem. Finally, we relate our work to Vainsencher's work with up to seven nodes.

==> corrections.tex <==
\magnification=\magstep1
\centerline{CORRECTIONS}
 \smallskip
\centerline{to be made to the article by S. Kleiman and R. Piene}
 \smallskip
\centerline{ENUMERATING SINGULAR CURVES ON SURFACES}
 \smallskip
\centerline{appearing in ``Algebraic geometry --- Hirzebruch 70,''}
 \smallskip
\centerline{{\it Cont. Math.} {\bf241} (1999), 209--238}

\bigskip

\def\nxt#1 {\medskip\noindent\hang p.\thinspace#1. --- \ignorespaces}

\nxt217b In the displayed formula for $\mathop{cod}({\bf D})$, replace
`$m_D$' by `$m_V$'.

\nxt219 In Table 2-1, the value of $r$ for $X_{1,2}$ should not be
1, but 4.

\nxt221b The proof of Proposition (3.2) should have used Gotzmann's
regularity theorem in much the same way that it is used in the proof of
Proposition~(3.5).  So replace the second paragraph in the first proof
by the following two.
 \newdimen\lskip \lskip=\hsize \advance\lskip by -5in
 {\smallskip \leftskip=\lskip
 There exists a map $\varphi$ from the germ of $Y$ at $y$ into $B$
carrying $y$ to the origin.  Since $m\ge\mu-1$ by hypothesis, $\varphi$ is
smooth, as we'll now show.  It suffices to show the surjectivity of the
map of tangent spaces, which is equal to the natural map,
    $$H^0({\cal L})/H^0({\cal O}_S)\to H^0\bigl({\cal L}\big/{\cal
K}_{C,S}{\cal L}\bigr).$$
 Since ${\cal N}$ is spanned, it suffices to show the surjectivity of the map,
  $$H^0({\cal M}^{\otimes m})\to
  H^0\bigl({\cal M}^{\otimes m}\!\big/{\cal K}_{C,S}{\cal M}^{\otimes
m}\bigr).\eqno(3.2.1)$$

To show the surjectivity of (3.2.1), embed $S$ in a projective space $P$
so that ${\cal M}={\cal O}_S(1)$, and let ${\cal K}_{C,P}\subset{\cal O}_P$
be the ideal such that
  $${\cal O}_P/{\cal K}_{C,P}={\cal O}_S/{\cal K}_{C,S}.$$
  Now,
since ${\cal K}_{C,S}\supset{\cal J}_{C,S}$, Proposition (3.1) implies that
        $\mu\ge\dim H^0({\cal O}_S/{\cal K}_{C,S})$.
 Hence, by Gotzmann's regularity theorem [{\bf 13}] (see also
[{\bf 14}, p.\thinspace80]), the ideal ${\cal K}_{C,P}$ is $\mu$-regular.  So
$H^1({\cal K}_{C,P}(m))$ vanishes for $m\ge \mu-1$.  Hence the map
	$$H^0({\cal O}_P(m))\to
         H^0\bigl(({\cal O}_P/{\cal K}_{C,P})(m)\bigr)$$
 is surjective.  It factors through (3.2.1), so (3.2.1) is surjective.
Thus $\varphi$ is smooth.
 \par}

\nxt225b In the third paragraph of the proof of (3.7), replace the third
sentence by the following one.
{\smallskip \leftskip=\lskip\noindent
  On the other hand, every fiber of $Z({\bf D})\to H({\bf D})$ is a
projective space, and meets $Z_0({\bf D})$ in a nonempty open subset by
(3.5).
 \par}

\nxt226m In the second paragraph of Section 4, replace the first clause
of the first sentence  by the following one.
{\smallskip \leftskip=\lskip\noindent
   Let $\pi\colon F\to Y$ be a smooth and projective family of (possibly
reducible) surfaces, where $Y$ is equidimensional and Cohen--Macaulay,
and \dots
 \par}

\nxt226m In the  displayed  sequence of principal parts, the the first
term should be twisted by $D$ too:
   $$0\to\mathop{\it Sym}\nolimits^{i-1}\Omega^1_{F/Y}(D)\to\cdots.$$
 
\nxt230t In (4.5), replace the final `$=$' by `$\le$', getting
	$$\dots\ a+b+2c\le r+2.\eqno(4.5) $$


 \nxt230m In the paragraph that begins, ``The genericity hypothesis also
implies,'' replace the first sentence by the following one.
 {\smallskip \leftskip=\lskip\noindent
 The genericity hypothesis also implies that $X_2$ is reduced,
Cohen--Macaulay, and equidimensional of codimension 3 in $F$.
 \par}

 \nxt231 In the second display, replace $w_1-e$ by $w_1+e$, and
$w_2+e^2$ by $w_2-e^2$.  In the third display, replace $w_1-e$ by $w_1+e$, and
$w_2+e$ by $w_2-e^2$.
 In the next to the last paragraph, replace $w_1-e$ by $w_1+e$ and
$w_2+e$ by $w_2-e^2$, and $w_2^3$ by $w_2e$. In the display, remove
$[X_i]$, and move the sentence following the display down to after the
next display.

 \nxt237 References 3, 4, 5, and 8 have appeared.  The bibliographic
data follows.
\frenchspacing
\smallskip
3. J. Amer. Math. Soc. {\bf13}(2) (2000), 371--410.

4. Duke Math. J. {\bf99}(2) (1999), 311--28.

5. Surveys in Diff. Geom. {\bf5} (1999), 313-39.

8. London Math Society Lecture Note Series {\bf276}, Cambridge
Univ. Press, 2000.

\bye

